Online Consistency of the Nearest Neighbor Rule

In the realizable online setting, a learner is tasked with making predictions for a stream of instances, where the correct answer is revealed after each prediction. A learning rule is online consistent if its mistake rate eventually vanishes. The nearest neighbor rule (Fix and Hodges, 1951) is a fundamental prediction strategy, but it is only known to be consistent under strong statistical or geometric assumptions: the instances come i.i.d. or the label classes are well-separated. We prove online consistency for all measurable functions in doubling metric spaces under the mild assumption that the instances are generated by a process that is uniformly absolutely continuous with respect to a finite, upper doubling measure.

==> figures/cover-tree-1.tex <==
\begin{tikzpicture}
    \def\boxsize{5}
    \def\ballsize{4.5}
    \def\area{(-\boxsize,-\boxsize) rectangle (\boxsize,\boxsize)}
    \def\cutout{(0,0) circle (\ballsize)}
    \draw[fill=white, draw=white] \area;  
    \clip[] (-4.7, -4.7) rectangle (4.7,4.7);

    \def\PointA{(-2,-1.5)}
    \def\PointB{(0,-0.75)} 
    \def\PointC{(0.6,2.3)}
    


    \begin{transparent}{0.5}
        \draw[fill=gradient0, draw=none] (0,0) circle (4.6); 
        \draw[fill=gradient1, draw=none] \PointA circle (6);
        \draw[fill=gradient2, draw=none] \PointA circle (3);
        \draw[fill=gradient3, draw=none] \PointA circle (1.5);
        \draw[fill=gradient4, draw=none] \PointA circle (0.75);   
        \draw[fill=gradient5, draw=none] \PointA circle (0.375);   
        \end{transparent}


    \draw[fill=black, draw=none] \PointA circle (0.07);


    \draw[fill=white, draw=none, even odd rule] \area \cutout;
\end{tikzpicture}%

==> figures/cover-tree-2.tex <==
\begin{tikzpicture}
    \def\boxsize{5}
    \def\ballsize{4.5}
    \def\area{(-\boxsize,-\boxsize) rectangle (\boxsize,\boxsize)}
    \def\cutout{(0,0) circle (\ballsize)}
    \draw[fill=white, draw=white] \area;  
    \clip[] (-4.7, -4.7) rectangle (4.7,4.7);

    \def\PointA{(-2,-1.5)}
    \def\PointB{(0,-0.75)} 
    \def\PointC{(0.6,2.3)}
    

    \begin{transparent}{0.5}
    \draw[fill=gradient0, draw=none] (0,0) circle (4.6); 
    \draw[fill=gradient1, draw=none] \PointA circle (6);
    \draw[fill=gradient2, draw=none] \PointA circle (3);
    \draw[fill=gradient3, draw=none] \PointA circle (1.5);
    \draw[fill=gradient4, draw=none] \PointA circle (0.75);   
    \draw[fill=gradient5, draw=none] \PointA circle (0.375);   
    \end{transparent}

    \begin{transparent}{0.5}
    \draw[fill=gradient3, draw=none] \PointB circle (1.5);
    \draw[fill=gradient4, draw=none] \PointB circle (0.75);
    \draw[fill=gradient5, draw=none] \PointB circle (0.375);
    
    \end{transparent}

    \draw[fill=black, draw=none] \PointA circle (0.07);
    \draw[fill=black, draw=none] \PointB circle (0.07);

    \draw[fill=white, draw=none, even odd rule] \area \cutout;
\end{tikzpicture}%

==> figures/cover-tree-3.tex <==
\begin{tikzpicture}
    \def\boxsize{5}
    \def\ballsize{4.5}
    \def\area{(-\boxsize,-\boxsize) rectangle (\boxsize,\boxsize)}
    \def\cutout{(0,0) circle (\ballsize)}
    \draw[fill=white, draw=white] \area;  
    \clip[] (-4.7, -4.7) rectangle (4.7,4.7);

    \def\PointA{(-2,-1.5)}
    \def\PointB{(0,-0.75)} 
    \def\PointC{(0.6,2.3)}
    

    \begin{transparent}{0.5}
    \draw[fill=gradient0, draw=none] (0,0) circle (4.6); 
    \draw[fill=gradient1, draw=none] \PointA circle (6);
    \draw[fill=gradient2, draw=none] \PointA circle (3);
    \draw[fill=gradient3, draw=none] \PointA circle (1.5);
    \draw[fill=gradient4, draw=none] \PointA circle (0.75);   
    \draw[fill=gradient5, draw=none] \PointA circle (0.375);   
    \end{transparent}

    \begin{transparent}{0.5}
    \draw[fill=gradient2, draw=none] \PointC circle (3);
    \draw[fill=gradient3, draw=none] \PointC circle (1.5);
    \draw[fill=gradient4, draw=none] \PointC circle (0.75);
    \draw[fill=gradient5, draw=none] \PointC circle (0.375);
    \end{transparent}

    \begin{transparent}{0.5}
    \draw[fill=gradient3, draw=none] \PointB circle (1.5);
    \draw[fill=gradient4, draw=none] \PointB circle (0.75);
    \draw[fill=gradient5, draw=none] \PointB circle (0.375);
    
    \end{transparent}

    \draw[fill=black, draw=none] \PointA circle (0.07);
    \draw[fill=black, draw=none] \PointC circle (0.07);
    \draw[fill=black, draw=none] \PointB circle (0.07);

    \draw[fill=white, draw=none, even odd rule] \area \cutout;
\end{tikzpicture}%

==> figures/gradients.tex <==
\definecolor{orange1}{RGB}{241, 229, 184}
\definecolor{orange2}{RGB}{230, 205, 140}
\definecolor{orange3}{RGB}{222, 180, 97}
\definecolor{orange4}{RGB}{215, 153, 56}
\definecolor{orange5}{RGB}{209, 124, 0}
\definecolor{orange0}{RGB}{224, 255, 255}
\definecolor{orange0}{RGB}{194, 244, 250}
